Adaptive Perturbation-Based Gradient Estimation for Discrete Latent Variable Models

The integration of discrete algorithmic components in deep learning architectures has numerous applications. Recently, Implicit Maximum Likelihood Estimation (IMLE, Niepert, Minervini, and Franceschi 2021), a class of gradient estimators for discrete exponential family distributions, was proposed by combining implicit differentiation through perturbation with the path-wise gradient estimator. However, due to the finite difference approximation of the gradients, it is especially sensitive to the choice of the finite difference step size, which needs to be specified by the user. In this work, we present Adaptive IMLE (AIMLE), the first adaptive gradient estimator for complex discrete distributions: it adaptively identifies the target distribution for IMLE by trading off the density of gradient information with the degree of bias in the gradient estimates. We empirically evaluate our estimator on synthetic examples, as well as on Learning to Explain, Discrete Variational Auto-Encoders, and Neural Relational Inference tasks. In our experiments, we show that our adaptive gradient estimator can produce faithful estimates while requiring orders of magnitude fewer samples than other gradient estimators.

==> algo-momentum.tex <==
\begin{algorithm*}[t]
\begin{multicols}{2}
%
\begin{algorithmic}
       \Function{Init}{$\alpha_{0}$, $\alpha_{m}$}
       \State $\alpha \leftarrow \alpha_{0}$ \quad // Initial value of $\alpha$
       \State $\overline{g} \leftarrow 1$ \quad // Initial gradient norm
       \State $\alpha_{s} \leftarrow \alpha_{s}$ // $\alpha$ update step
       \State $\alpha_{m} \leftarrow \alpha_{m}$ \quad // $\alpha$ update momentum
       \EndFunction
       
       \item[]
       \item[]
       
       \Function{Forward}{$\btheta$}
       \State // Sample from the noise distribution $\rho(\bepsilon)$
       \State $\bepsilon_{1}, \ldots, \bepsilon_{N} \sim \rho(\bepsilon)$
       \State // MAP state of perturbed $\btheta$
       \State $\exz_{i} \leftarrow \fMAP(\btheta + \bepsilon_{i})$, for $i = 1, \ldots, N$
       %\State $\exz_{2} = \fMAP(\btheta + \bepsilon_{2})$
       \Save $\btheta$, $\bepsilon_{1, \ldots, N}$, and $\exz_{1, \ldots, N}$ % for the backward pass
       \Return $\exz_{1, \ldots, N}$
       \EndFunction
       
       \item[]
       \item[]
       
\end{algorithmic}
%
\begin{algorithmic}
       \Function{Backward}{$\grad{\bz}{\ell}(f_{\bu}(\bz_{1, \ldots, N}), \exy)$}
       \Load $\btheta$, $\bepsilon_{1, \ldots, N}$, and $\exz_{1, \ldots, N}$ %from the forward pass
       
       \State $\lambda = \alpha \frac{ \norm{\btheta}_{2} }{ \norm{\grad{\bz}{\ell}(f_{\bu}(\bz_{1, \ldots, N}), \exy)}_{2} }$ (see \cref{eq:lambda})
       
       \State // Target distribution parameters
       
       %\State $\btheta_{R}' = \btheta - \lambda \grad{\bz}{\ell}(f_{\bu}(\bz_{1}), \exy)$
       
       \For{$i = 1, \ldots, N$}
       
           \State $\btheta_{R_{i}}' \leftarrow \btheta - \lambda \grad{\bz}{\ell}(f_{\bu}(\exz_{i}), \exy)$
           \State $\btheta_{L_{i}}' \leftarrow \btheta + \lambda \grad{\bz}{\ell}(f_{\bu}(\exz_{i}), \exy)$
           
           %\\ \Comment{Single sample \imle gradient estimates}
           
           \State $g_i \leftarrow \frac{1}{2} \left[ \fMAP(\btheta_{L_{i}}' + \bepsilon_{i}) - \fMAP(\btheta_{R_{i}}' + \bepsilon_{i}) \right]$
       \EndFor
       
       \State // Running estimate of the gradient norm
       \State $\overline{g} \leftarrow 0.9 \ \overline{g} + 0.1 \ \frac{1}{N} \sum_{i = 1}^{N} \norm{g_{i}}_{0}$
       
       \State // Increase $\alpha$ using momentum until $\overline{g} \approx c$
       %\State $\alpha \leftarrow \alpha + \begin{cases} \eta & \text{if } \overline{g} < c \\ - \eta & \text{otherwise}\end{cases}$
       \State $\alpha_{u} \leftarrow \alpha_{m} \ \alpha_{u} + \left( \alpha_{s} \text{ if } \ \overline{g} < c \ \text{else} - \alpha_{s} \right)$
       \State $\alpha \leftarrow \left[ \alpha + \alpha_{u} \right]_{+}$
       
       %\State $g = (g_1 + g_2) / 2.0$
       %\State $g = \frac{1}{N}\sum_{i = 1}^{N} g_{i}$
       %\State $\mlegradient(\extheta, \extheta') = \fMAP(\btheta_{L}' + \bepsilon) - \fMAP(\btheta_{R}' + \bepsilon)$
       %\State $\gamma \leftarrow 0.9 \gamma + 0.1 \norm{\mlegradient(\extheta, \extheta')}_{0}$
       %\If{$\gamma < 1.0$}
       %\State $\beta = \beta + 0.001$ 
       %\Else
       %\State $\beta = \beta - 0.001$
    %    \EndIf
       %\Return $g$ %$\mlegradient(\extheta, \extheta')$
       \Return $\frac{1}{N}\sum_{i = 1}^{N} g_{i}$
       \EndFunction
\end{algorithmic}
\end{multicols}
\caption{Two-sided, adaptive, and perturbation-based \imle.}
% as a layer.
\label{algo:main}
\end{algorithm*}


==> tables/dvae_tab.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.48\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/dvae-tab/DVAE_IMLE_1-crop.pdf}
  \caption{A subfigure}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/dvae-tab/DVAE_IMLE_10-crop.pdf}
  \caption{A subfigure}
  \label{fig:sub2}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:dvae1}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{.48\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/dvae-tab/DVAE_STE_1-crop.pdf}
  \caption{A subfigure}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/dvae-tab/DVAE_STE_10-crop.pdf}
  \caption{A subfigure}
  \label{fig:sub2}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:dvae1}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{.48\linewidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/dvae-tab/DVAE_GS_1-crop.pdf}
  \caption{A subfigure}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/dvae-tab/DVAE_GS_10-crop.pdf}
  \caption{A subfigure}
  \label{fig:sub2}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:dvae2}
\end{figure*}


==> tables/synth_lambdas.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.48\linewidth}
  \centering
  % \includegraphics[width=1\linewidth]{figures/synth/gradient_20_1_128.pdf}
  \includegraphics[width=1\linewidth]{figures/synth/v9/gradient_s=1000_n=30_k=1_w=10000_m=0.0_t=1.pdf}
  \caption{A subfigure}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  %\includegraphics[width=1\linewidth]{figures/synth/gradient_50_1_128.pdf}
  \includegraphics[width=1\linewidth]{figures/synth/v9/gradient_s=1000_n=50_k=1_w=10000_m=0.0_t=1.pdf}
  \caption{A subfigure}
  \label{fig:sub2}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:synth}
\end{figure*}


